SketchGen: Generating Constrained CAD Sketches

Computer-aided design (CAD) is the most widely used modeling approach for technical design. The typical starting point in these designs is 2D sketches which can later be extruded and combined to obtain complex three-dimensional assemblies. Such sketches are typically composed of parametric primitives, such as points, lines, and circular arcs, augmented with geometric constraints linking the primitives, such as coincidence, parallelism, or orthogonality. Sketches can be represented as graphs, with the primitives as nodes and the constraints as edges. Training a model to automatically generate CAD sketches can enable several novel workflows, but is challenging due to the complexity of the graphs and the heterogeneity of the primitives and constraints. In particular, each type of primitive and constraint may require a record of different size and parameter types. We propose SketchGen as a generative model based on a transformer architecture to address the heterogeneity problem by carefully designing a sequential language for the primitives and constraints that allows distinguishing between different primitive or constraint types and their parameters, while encouraging our model to re-use information across related parameters, encoding shared structure. A particular highlight of our work is the ability to produce primitives linked via constraints that enables the final output to be further regularized via a constraint solver. We evaluate our model by demonstrating constraint prediction for given sets of primitives and full sketch generation from scratch, showing that our approach significantly out performs the state-of-the-art in CAD sketch generation.

==> bnf.tex <==
%-----cut here with a sharp machete or an 19.95 ginsu knife
%************************************************************************
%* BNF.tex								*
%* 									*
%* plain tex macros for formatting grammars				*
%*									*
%* Erik Quanstrom 							*
%* 10. November 1990							*
%************************************************************************

%things to fix:
%	make configurable
%	work with texinfo

\gdef\actifygrammarchars{%
	\catcode`\>\active%
	\catcode`\<\active%
	\catcode`\:\active%
	\catcode`\"\active%
	\catcode`\;\active%
	\catcode`\.\active%
	\catcode`\|\active%
	\catcode`\,\active}

\gdef\deactifygrammarchars{%
	\catcode`\>12%
	\catcode`\<12%
	\catcode`\:12%
	\catcode`\;12%
	\catcode`\.12%
	\catcode`\|12%
	\catcode`\,12}

\newif\ifquote
\quotefalse

\begingroup
   \actifygrammarchars
   \gdef>{\/\endgroup$\rangle$\relax}
   \gdef<{$\langle$\begingroup\sl}
   \gdef:{$\rightarrow$}

   \begingroup
	\catcode`\"\active
	\gdef"{\ifquote%
		'\endgroup\quotefalse%
	   \else%
		\quotetrue\begingroup\deactifygrammarchars\bf`%
	\fi}%
   \endgroup

   \gdef;{\hfill\break}
   \gdef.{\relax}
   \gdef|{$\vert$}
   \gdef,{;\hbox to 1cm{\hfill}}
\endgroup

\def\begingrammar{%
	\begingroup
	\advance\leftskip by 1cm%
	\parindent=-1cm%
	\actifygrammarchars%
	\def\endgrammar{\endgroup}
	\parskip 1ex%
	\relax
}

%
%
%
\def\ul{\lower .2ex\hbox to 1ex{\hrulefill}\relax}%



==> sections/checklist.tex <==
% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We claim a new language for CAD sketches that improves upon the state-of-the art in CAD sketch generation. We empirically show the claimed improvements in Section~\ref{sec:results}.}
  \item Did you describe the limitations of your work?
    \answerYes{Section~\ref{sec:conclusion} describes several limitations of our work. In addition, we discuss failure cases in the supplementary material.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We describe these in the supplementary material.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
    \end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{The paper is empirical with no theoretical results.}
    \item Did you include complete proofs of all theoretical results?
    \answerNA{We do not present any proofs.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We will provide an early version of our code in the supplementary material, and will publish a cleaner version closer to the conference date.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In Section \ref{sec:results}, we describe the dataset processing scheme and our hyperparameters for our models. We have the complete architectural details in the Supplementary material}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{This is reported in Section \ref{sec:results}}
    \end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We provide a citation \cite{SketchGraphs}}
  \item Did you mention the license of the assets?
    \answerYes{We mention the license of the dataset we use in Section~\ref{sec:results}, paragraph `Dataset'.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{We introduced no assets}
    \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> sections/old_text.tex <==
%\paragraph{Quantitative comparison} The basic metric for assessing the generative capability of the model is the Negative Log-Likelihood, which we report in the average number bits required to represent a token, a single primitive or a single instance. We additionally report the accuracy which is the rate at which the Primitive model is able to predict the next token in the sequence given the current partial sequence. For measuring both of these metrics, we mask out all tokens after the stop token. which are added to pad small sequences to a maximum sequence length. As we perform minimal masking on the output probabilities of then network, the network can also produce sequences that do no follow our grammar, and cannot be parsed into primitives. Thus, we also report the  fraction of generated samples that are valid under our grammar. These metrics are how we assess \textbf{syntactic metrics} of our model. 
%We additionally need to measure how close the generated sketches are to actual CAD models from the training set. We refer to these quantities as the \textbf{semantic metrics}. These are measured on a distributional level over the whole generated samples, and quantify on an aggregate level the geometric properties of our generated sketches. These are \wamiq{Choose which ones to report}

% \paragraph{Qualitative comparison}

% \begin{table}[h]
% \caption{Comparison on primitive sequences. }
% \centering 
% \small
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{lcccccc} 
% \toprule
% & \multicolumn{3}{c}{Syntactic} & Semantic \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-5}
% Method & Bits/token & Bits/Primitive & Bits/Sequence & Accuracy & Parseable & EMD \\
% \midrule \midrule
% SketchGraphs & uu & vv & ww & xx & yy & zz  \\
% % Autodesk & uu & vv & ww & xx & yy & zz \\
% Ours (p=1.0) & uu & vv & ww & xx & yy & zz \\
% Ours (p=0.9) & uu & vv & ww & xx & yy & zz \\
% Ours (optimized) & uu & vv & ww & xx & yy & zz \\

% \bottomrule
% \end{tabular}
% \label{tab:prim_metrics}
% \end{table}

% \begin{figure}[h]
%     \small
%     \begin{subfigure}{.23\textwidth}
%       \centering
%       % include first image
%       \includegraphics[width=\textwidth]{example-image}
%       \caption{x-line directions}
%     \end{subfigure}
%     ~
%     \begin{subfigure}{.23\textwidth}
%       \centering
%       % include first image
%       \includegraphics[width=\textwidth]{example-image}
%       \caption{y-line directions}
%     \end{subfigure}
%     ~
%     \begin{subfigure}{.23\textwidth}
%       \centering
%       % include first image
%       \includegraphics[width=\textwidth]{example-image}
%       \caption{circle radii}
%     \end{subfigure}
%     ~
%     \begin{subfigure}{.23\textwidth}
%       \centering
%       % include first image
%       \includegraphics[width=\textwidth]{example-image}
%       \caption{kde of prim counts}
%     \end{subfigure}
%     ~
%     \caption{(Semantic quality) Distributions of sampled vs GT primitive quanitites.}
%     \label{fig:sketch_gen}
% \end{figure}


% \begin{itemize}

% \item Baselines: Model that was introduced with dataset
% \item Metrics: Statistics, NLL
% \item Qualitative: ~ 10-20 examples
% \end{itemize}

%, and the \emph{primitive accuracy} (($A^P$), measured as the accuracy of primitive parameters

%We include an additional baseline, where coincidence constraints are generated by 

%As another generative model, we assess the generative capability of our model with the Negative Log-Likelihood reported here in the average bits/token,  bits/constraint and bits/sequence. Syntactical metrics measured are the accuracy of next token generation and the ratio of sequences with valid syntax. An additional metric we report is the Constraint Accuracy - given a test sample with ground truth constraints available, we run our Constraint Model and infer the constraints. The Constraint Accuracy is then the ratio of correctly predicted constraints to the total number of predicted constraints. We also report the Precision (P) and Recall (R) of our predicted constraints over the test set.

% Semantic metrics for constraints are also computed on a distribution level. \wamiq{Report what we measure}

%that takes as input the feature vector $f_i$ and outputs the next token $q_i$ in the sequence $Q$. 
%training time: teacher forcing

%inference time: determine syntax of primitive or constraints tree based on generated primitive type $\tau$ or constraint type $\nu$, as shown in Figure~\ref{fig:generation}.

%limit generated token values to valid range for the given token using the known syntax. For example, correct generated values for tokens $\alpha$ and $\omega$ to the expected special values if a different value has not been generated.

% \begin{itemize}
%     \item  We first translate all sketches, so the origin is at the center of their bounding boxes and scale them to a uniform size.
%     \item  We have the following primitives - point, line, circle, arc. The primitives each have certain parameters. We quantize all parameters with the following strategy - we collect shared params eg x/y is present in all primitives, a radius in circle/arc.
%     \item  We then perform k-means clustering on each of the parameter groups and quantize. Uniformly quantizing is wasteful as some directions (or other parameters ) are over-represented (horiz/vertical/45 degree). Not quantizing all param groups with the same dictionary is also important as paramter groups have different ranges, angles will always be between 0-360, while radii span a range 0-10, in our -5 to 5 rescaling.
%     \item  We create a structured variable length sequence by introducing a break between different primitives by using an additional padding token. The first token is the \textsc{PrimitiveID} token which identifies the nature of the rest of the sequence until the new padding token.
%     \item During training, we give these tokens - the parameter tokens of the prims that build the sketch with a start and stop token, and the intermediate padding \textsc{NewPrim} token, the position token, for each prim, each of its parameter token has the tokens of \textsc{PrimitiveType}, and within each primitive we provide additional information by having a \textsc{ParameterType} token - eg x/y within all primitives will share this token, same with radii etc.
%     \item Trained with teacher forcing to maximize log-likelihood.
%     \item During sampling, we start with the \textsc{Start} token. The \textsc{PrimitiveType} and \textsc{ParameterType} get a special \textsc{Pad} value. Depending on the next token sampled, we change the \textsc{PrimitiveType} and \textsc{ParamterType} token at every sampling step. The \textsc{PrimitiveType} stays the same until the 
%     \textsc{NewPrim} token is generated. The \textsc{ParamterType} token depends on the type of the initial token that was generated which determines the primitive type.
%     \item The sampling may not generate the \textsc{NewPrim} token even when the parameters of the primitive are exhausted. We force the sampler to generate a \textsc{NewPrim} token in that case.
% \end{itemize}



%is a common problem with rule-based methods, which need significant post-processing to prune the large set of discovered constraints.
%  that they require 

% In order to establish a baseline to compare our constraint generation capability, we infer constraints using simple rules. As an example, to identify a \texttt{CoincidenceConstraint} amongst two lines, we check if their end points are within an $\epsilon$ distance of one another. Notice that existing CAD modelling software already implements this, but we found in our experience that it is a significant effort to write custom implementations for each constraint, and as the rules are custom require significant tuning of parameters. We compare this baseline to our constraint generation method in Figure \ref{fig:snapping}. We see that the snappping baseline over-estimates the number of coincidences significantly with $\epsilon=0.03$ and $\epsilon=0.1$. This is a common problem with rule-based methods that they require significant post-processing to prune the large set of discovered constraints.



%Generate constraints on existing primitives from testset (quantized and optionally with added noise) and optimize primitives with generated constraints


% \begin{itemize}
% \item Baselines: Model that was introduced with dataset (can this model generate constraints only?), snapping baseline
% \item Metrics: Statistics of constraints, NLL, Constraint Accuracy
% \item Qualitative: ~ 10-20 examples, each before+after optimization with the generated constraints
% \end{itemize}

% \begin{figure}[h]
%     \small
%     \begin{subfigure}{.23\textwidth}
%       \centering
%       % include first image
%       \includegraphics[width=\textwidth]{example-image}
%       \caption{loc of coincidence}
%     \end{subfigure}
%     ~
%     \begin{subfigure}{.23\textwidth}
%       \centering
%       % include first image
%       \includegraphics[width=\textwidth]{example-image}
%       \caption{loc of tangency}
%     \end{subfigure}
%     ~
%     \begin{subfigure}{.23\textwidth}
%       \centering
%       % include first image
%       \includegraphics[width=\textwidth]{example-image}
%       \caption{subnode kde coinc.}
%     \end{subfigure}
%     ~
%     \begin{subfigure}{.23\textwidth}
%       \centering
%       % include first image
%       \includegraphics[width=\textwidth]{example-image}
%       \caption{kde of constr counts}
%     \end{subfigure}
%     ~
%     \caption{(Semantic quality) Distributions of sampled vs GT primitive quanitites.}
%     \label{fig:my_label}
% \end{figure}

% \subsection{Conditional Generation}
% Only if time allows: Generate conditioned on image similar to Deepmind paper


%\paragraph{Primitive Model} We begin to remove the additional tokens induced by our grammar. The results are shown in Table \ref{tab:ablation_prim}. There are three variants - Baseline which is our model with all the tokens embedded during training. The second model is B - $Q^3$ where we remove the $Q^3$ tokens during training. Removing this token causes the performance of the model to degrade slightly. The third variant is B - $Q^3$ - $Q^4$, where we remove both $Q^3$ and $Q^4$ tokens during training. This causes a significant drop in performance of with the model taking 0.4 more bits to represent a sequence. 


% \paragraph{Constraint Model} We perform a similar task on the Constraint Model. We ablate on three design choices: 1) We remove the tokens generated by our grammar on the constraint sequences. This is the B- $Q^4$ model 2) In the B-\texttt{shared} model, we see the effect of having a shared embedding dictionary for the primitive parameter tokens. Instead of sharing same dictionary (Equation \ref{eq:pointer_prim_encoding}) for each parameter, we choose an arbitrary but fixed dictionary to embed parameters into. For example, location parameters of a line would share a common dictionary with the angle parameters of an arc. For the actual sharing scheme, see the Supplementary. 3. Additionally, we hypothesized that we could offset error introduced by our quantization scheme by jittering primitive tokens during training to make the network more robust. During training, we added Bernoulli noise to the location parameters of each of the primitives with a probability 0.25. The magnitude of the noise is $1/256$, ie we jitter by one bin width if quantization was uniform. This model is called B +\texttt{perturb}. The results are shown in Table \ref{tab:ablation_constraint}. We see again the careful encoding is very important to achieve good performance. Removal of $Q^4$, which is added to the constraint sequence is equally as catastrophic as not having a good encoding scheme for the primitives, as shown by removal of \texttt{shared} embeddings. Surprisingly, adding jitter led to worse modelling performance. This means the network itself is capable of correcting for errors introduced due to the quantization of primitive parameters. 


\section{Notes}
\subsection{Special Instructions}
\begin{enumerate}
    \item This years NIPS submissions are 9 pages long with a smaller margin on the sides so we have more text to fill in than usual
    \item All submissions need a checklist of ethics/reproducibility/etc. Please check \verb+sections/checklist.tex+
    \item One of the checklist items is providing error bars by averaging across multiple runs, so we need tons of runs.
    \item If we conduct a user-study, we also need to completely describe the user study (and report how much we paid them?)
    \item The supplementary submission deadline is June 2.
\end{enumerate}

\subsection{Plan/Progress}
\begin{enumerate}
    \item The first thing to do is extensively verify and re-verify results.
    \item This is what I consider the constributions of the method:
        \begin{enumerate}
            \item Showing that primitives can be generated by a transformer - primitives  are variable length sequences within variable length sequences.
            \item This generation is possible with quantizing the continuous variables
            \item Furthermore, we can take this list of quantized prims and infer constraints from them, recovering constrained CAD geometry of high quality.
            \item \textit{TBD} If we have access to a black-box geometry solver, we can also \textit{fix} the bad primitives byb passing them in along with the inferred constraints
        \end{enumerate}
    \item The main challenge still is the evaluation. Current quantitative TODO:
        \begin{enumerate}
            \item NLL of the primitives. NLL of constraints.
            \item NLL comparison to SketchGraphs.
            \item Accuracy of constraint sequence - take validation prims, infer constraints, see how many we get right.
            \item Primitive quality. These are done on a distribution level instead of per instance. Right now we measure simple stats - number of prims per instance. Need to add: a histogram of line directions, line lengths, circle centers and radii, arc sweep angles and centers.
            \item To measure instance quality, we have to measure how prims interact. Ideally there would be higher level metrics - how many loops there are? how many motifs, eg a chamfer next to a hole is very very common, or chamfers with arc ending on two stright face. This I think is itself another project, so we stick to basic stuff. We consider pairs of prims and measure how they interact. ie we compute stats on
            \begin{enumerate}
                \item coincidence constraint: histograms of where do coincidences occur, what prims do they involve, what parts of those prims do they involve
                \item tangency constraint: histogram of which circles are involved in tangency - where are their centers, what are their radii. At what angle do the lines that are tangent exist.
                \item parallel/vertical/horizontal: same stuff
                \item In addition we also compute the number of such constraints per instance
            \end{enumerate}
            \item Compare all of this to the dataset itself, and SketchGraphs.
        \end{enumerate}
    \item Ablations
        \begin{enumerate}
            \item Different quantization levels - 8-bit and 9-bit are standard. We can show a lot of degradation by going lower. And with 10 bits, we essentially have a 1000-class classification problem, which I hope would be too difficult to the net.
            \item Different quantization/encoding strategies - currently we quantize the paramterization itself meaning the x/y are quantized but so are the directions. Would it make more sense to represent all prims as points in a canonical order - eg line is two points, circle two (if along x-axis), arc three. Then the quantization would proably not be as disruptive. Will that aid prim quality?
            \item Different quantization strategy - I did an experiment way back where each primitives stats were used only to quantize that primitive meaning to quantize x/y of circles kmeans was run on x/y of all circles instead of all prims. That worked way worse - I think a) because of less data per prim for kmeans b) low correlation between indices of different prims giving the transformer a harder time.
        \end{enumerate}
        
    \item Fancy renderings and comparisons
        \begin{enumerate}
            \item One nice thing we can do is if we can extrude generated geometry and render it - it looks very slick
            \item In the best case, we can have three comparisons - to the dataset paper (which is mandatory), to the Google+Onshape paper, and to the Autodesk paper.
            \item To compare to the Google paper, we would need a sketch->CADModel transformer, and ask them for code.
            \item To compare to the Autodesk paper, we would also need to ask them for code, and possibly retrain as they use a different split compared to us.
        \end{enumerate}
    
\end{enumerate}


\begin{minipage}[h]{0.48\textwidth}
    \caption{
    Ablation on the constraint model.
    % $Q^4$ refers to the additional tokens describing the sequence, as discussed in Section \ref{fig:grammar}. \texttt{shared} means that primitive tokens of different types are embedded into separate dictionaries. \texttt{perturb} means the location coordinates are jittered during training.
    }
    \centering 
    \small
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{lccc} 
    \toprule
    method & NLL/seq. & NLL/constr. & Accuracy \\
    \midrule \midrule
    ours & xx & 8.28 & 97.4 \\
    ours -$Q^4$ & xx & 8.47 & 97.4 \\
    ours -\texttt{shared} & xx & 8.45 & 97.3\\
    % B +\texttt{perturb} & 8.43 & 97.4 \\
    \bottomrule
    \end{tabular}
    \label{tab:ablation_constraint}

% \end{table/}
\end{minipage}

